CrossCodeBench: Benchmarking Cross-Task Generalization of Source Code Models

Despite the recent advances showing that a model pre-trained on large-scale source code data is able to gain appreciable generalization capability, it still requires a sizeable amount of data on the target task for fine-tuning. And the effectiveness of the model generalization is largely affected by the size and quality of the fine-tuning data, which is detrimental for target tasks with limited or unavailable resources. Therefore, cross-task generalization, with the goal of improving the generalization of the model to unseen tasks that have not been seen before, is of strong research and application value. In this paper, we propose a large-scale benchmark that includes 216 existing code-related tasks. Then, we annotate each task with the corresponding meta information such as task description and instruction, which contains detailed information about the task and a solution guide. This also helps us to easily create a wide variety of ``training/evaluation'' task splits to evaluate the various cross-task generalization capabilities of the model. Then we perform some preliminary experiments to demonstrate that the cross-task generalization of models can be largely improved by in-context learning methods such as few-shot learning and learning from task instructions, which shows the promising prospects of conducting cross-task learning research on our benchmark. We hope that the collection of the datasets and our benchmark will facilitate future work that is not limited to cross-task generalization.

==> tables/results_overall_old.tex <==
\begin{table*}[t!]
    \centering
    \caption{Overall Benchmarking Results}
    \label{table:results_overall}
    \resizebox{\linewidth}{!}{%
    \begin{NiceTabular}{lllr|rr|r|rr|r|rr|r|rr|rr|rr}
        \CodeBefore
            \cellcolor{gray!15}{6-2,6-3,6-4,6-5,6-6,6-7,6-8,6-9,6-10,6-11,6-12,6-13,6-14,6-15,6-16,6-17,6-18,6-19}
            \rowcolors{7}{}{gray!15}[cols=3-19]
        \Body
            \toprule
                \Block{4-1}{\textbf{Type}} &
                \Block{4-1}{\textbf{Models}} &
                \Block{4-1}{\textbf{Methods}} &
                \Block{1-6}{\textbf{Cross-Category}} &
                &
                &
                &
                &
                &
                \Block{1-6}{\textbf{Cross-Sub-Type}} &
                &
                &
                &
                &
                &
                \Block{1-4}{\textbf{Cross-Type}} &
                &
                &
                \\
            \cline{4-19}
                &
                &
                &
                \Block{1-3}{\textbf{Intra}} &
                &
                & 
                \Block{1-3}{\textbf{Inter}} &
                &
                & 
                \Block{1-3}{\textbf{Intra}} &
                &
                &
                \Block{1-3}{\textbf{Inter}} &
                &
                &
                &
                &
                &
                \\
            \cline{4-19}
                &
                &
                &
                \Block{}{\textbf{CD}} &
                \Block{1-2}{\textbf{BF}} &
                &
                \Block{}{\textbf{CD}} &
                \Block{1-2}{\textbf{BF}} &
                &
                \Block{}{\textbf{ML}} &
                \Block{1-2}{\textbf{C2T}} &
                &
                \Block{}{\textbf{ML}} &
                \Block{1-2}{\textbf{C2T}} &
                &
                \Block{1-2}{\textbf{Trans}} &
                &
                \Block{1-2}{\textbf{QA}} &
                \\
            \cline{4-19}
                &
                &
                &
                \textbf{EM} &
                \textbf{B.} &
                \textbf{R.L} &
                \textbf{EM} &
                \textbf{B.} &
                \textbf{R.L} &
                \textbf{EM} &
                \textbf{B.} &
                \textbf{R.L} &
                \textbf{EM} &
                \textbf{B}. &
                \textbf{R.L} &
                \textbf{B.} &
                \textbf{R.L} &
                \textbf{B}. &
                \textbf{R.L} \\
            \midrule
                \Block{2-1}{Shortcut} &
                \Block{1-2}{Copy Ex-output} &
                &
                \textbf{50.00} &
                10.35 &
                20.24 &
                50.00 &
                10.35 &
                20.24 &
                \textbf{10.75} &
                2.52 &
                1.43 &
                10.75 &
                2.52 &
                1.43 &
                3.97 &
                15.95 &
                3.29 &
                2.71 \\
            &
                \Block{1-2}{Copy Ins-input} &
                &
                0.00 &
                40.51 &
                54.59 &
                0.00 &
                40.51 &
                54.59 &
                0.00 &
                1.28 &
                3.55 &
                0.00 &
                1.28 &
                3.55 &
                45.44 &
                60.67 &
                0.82 &
                2.00 \\
            \hline
                \Block{7-1}{Off-the-\\Shelf} &
                \Block{5-1}{OPT} &
                4-shot &
                1.09 &
                19.88 &
                20.17 &
                1.09 &
                19.88 &
                20.17 &
                0.05 &
                2.51 &
                2.29 &
                0.05 &
                2.51 &
                2.29 &
                14.02 &
                23.34 &
                5.35 &
                7.82 \\
            &             
                & 
                3-shot &
                0.58 &
                18.18 &
                19.59 &
                0.58 &
                18.18 &
                19.59 &
                0.00 &
                1.41 &
                1.04 &
                0.00 &
                1.41 &
                1.04 &
                12.56 &
                21.49 &
                5.06 &
                7.12 \\
            &
                & 
                2-shot &
                0.21 &
                17.08 &
                18.87 &
                0.21 &
                17.08 &
                18.87 &
                0.00 &
                1.39 &
                1.26 &
                0.00 &
                1.39 &
                1.26 &
                11.12 &
                20.90 &
                4.17 &
                6.84 \\
            &             
                & 
                1-shot &
                0.07 &
                16.25 &
                16.20 &
                0.07 &
                16.25 &
                16.20 &
                0.00 &
                0.89 &
                0.55 &
                0.00 &
                0.89 &
                0.55 &
                8.42 &
                18.95 &
                4.94 &
                5.98 \\
            &             
                & 
                zero-shot &
                0.00 &
                9.23 &
                9.99 &
                0.00 &
                9.23 &
                9.99 &
                0.00 &
                0.94 &
                0.98 &
                0.00 &
                0.76 &
                0.63 &
                5.66 &
                13.63 &
                3.64 &
                4.39 \\
            \cline{2-19}
                & 
                \Block{2-1}{Tk-\\Instruct} & 
                2/0-instruct &
                2.96 &
                29.91 &
                33.23 &
                2.96 &
                29.91 &
                33.23 &
                0.12 &
                3.58 &
                3.97 &
                0.12 &
                3.58 &
                3.97 &
                17.31 &
                29.87 &
                9.11 &
                8.94 \\
            &             
                & 
                2/2-instruct &
                2.22 &
                29.65 &
                32.45 &
                2.22 &
                29.65 &
                32.45 &
                0.11 &
                3.66 &
                3.42 &
                0.11 &
                3.66 &
                3.42 &
                16.46 &
                29.27 &
                8.10 &
                8.38 \\
            \hline
                \Block{16-1}{Fine-\\Tuned} & 
                \Block{7-1}{PLBART} &
                4-shot &
                15.86 &
                44.76 &
                57.52 &
                25.54 &
                55.86 &
                67.89 &
                1.75 &
                7.92 &
                6.61 &
                8.54 &
                11.95 &
                12.84 &
                50.14 &
                63.84 &
                12.37 &
                14.61 \\
            &
                & 
                3-shot &
                12.94 &
                43.60 &
                56.40 &
                23.49 &
                54.38 &
                65.21 &
                1.23 &
                7.58 &
                6.65 &
                5.82 &
                11.61 &
                11.59 &
                47.90 &
                62.35 &
                11.86 &
                13.59 \\
            &
                & 
                2-shot &
                10.59 &
                40.84 &
                54.37 &
                22.01 &
                49.73 &
                64.79 &
                0.89 &
                5.44 &
                5.54 &
                3.74 &
                10.73 &
                11.12 &
                47.60 &
                60.76 &
                9.61 &
                11.70 \\
            &
                &
                1-shot &
                9.27 &
                36.45 &
                46.90 &
                21.95 &
                45.95 &
                54.78 &
                0.56 &
                5.86 &
                4.03 &
                3.12 &
                10.51 &
                10.78 &
                46.66 &
                59.83 &
                8.84 &
                9.86 \\
            &
                &
                zero-shot &
                7.65 &
                45.36 &
                44.08 &
                16.40 &
                52.04 &
                50.34 &
                0.03 &
                3.66 &
                3.61 &
                2.81 &
                7.63 &
                6.87 &
                41.48 &
                54.31 &
                6.99 &
                8.33 \\
            &
                &
                2/0-instruct &
                19.11 &
                47.74 &
                59.23 &
                53.25 &
                59.19 &
                70.55 &
                4.82 &
                8.18 &
                7.22 &
                14.66 &
                14.31 &
                15.43 &
                48.88 &
                65.70 &
                15.72 &
                18.73 \\
            &
                &
                2/2-instruct &
                19.86 &
                42.84 &
                57.74 &
                53.87 &
                58.80 &
                68.89 &
                4.76 &
                8.96 &
                7.82 &
                14.82 &
                14.16 &
                14.24 &
                47.43 &
                63.95 &
                15.37 &
                17.76 \\
            \cline{2-19}
                &
                \Block{7-1}{CodeT5} &
                4-shot &
                15.80 &
                46.89 &
                58.15 &
                30.03 &
                56.92 &
                72.01 &
                1.80 &
                7.38 &
                6.80 &
                8.30 &
                12.15 &
                12.04 &
                49.22 &
                66.26 &
                14.78 &
                15.12 \\
            &
                &
                3-shot &
                13.05 &
                44.67 &
                57.33 &
                29.55 &
                54.30 &
                69.41 &
                1.04 &
                7.84 &
                6.59 &
                6.83 &
                11.49 &
                10.06 &
                47.83 &
                64.35 &
                14.27 &
                14.99 \\
            &
                &
                2-shot &
                12.49 &
                40.94 &
                52.68 &
                29.53 &
                51.26 &
                62.70 &
                0.81 &
                6.88 &
                5.85 &
                3.47 &
                10.50 &
                10.46 &
                48.65 &
                65.25 &
                13.69 &
                14.73 \\
            &
                &
                1-shot &
                10.68 &
                35.32 &
                45.38 &
                28.75 &
                48.86 &
                58.14 &
                0.34 &
                6.37 &
                5.57 &
                2.78 &
                9.87 &
                8.47 &
                45.72 &
                62.92 &
                11.41 &
                12.25 \\
            &
                &
                zero-shot &
                7.12 &
                30.69 &
                43.07 &
                18.8 &
                45.85 &
                56.51 &
                0.05 &
                4.15 &
                3.72 &
                1.95 &
                6.44 &
                6.99 &
                43.24 &
                58.38 &
                9.12 &
                10.95 \\
            &
                &
                2/0-instruct &
                20.89 &
                \textbf{48.33} &
                \textbf{61.02} &
                56.33 &
                \textbf{61.89} &
                \textbf{76.89} &
                5.57 &
                8.35 &
                7.10 &
                \textbf{15.95} &
                15.40 &
                15.63 &
                \textbf{52.05} &
                \textbf{67.87} &
                \textbf{17.95} &
                20.52 \\
            &
                &
                2/2-instruct &
                20.05 &
                45.57 &
                59.31 &
                \textbf{56.42} &
                58.49 &
                74.26 &
                5.06 &
                8.05 &
                6.93 &
                15.10 &
                14.60 &
                \textbf{15.90} &
                51.51 &
                66.61 &
                17.31 &
                20.12 \\
            \cline{2-19}
                &
                \Block{2-1}{Tk-\\Instruct} &
                2/0-instruct &
                18.43 &
                43.86 &
                57.23 &
                51.88 &
                57.45 &
                70.98 &
                4.92 &
                \textbf{9.18} &
                \textbf{8.47} &
                15.64 &
                \textbf{15.60} &
                14.35 &
                45.49 &
                62.14 &
                17.04 &
                \textbf{20.67} \\
            &
                &
                2/2-instruct &
                18.52 &
                42.01 &
                56.16 &
                51.20 &
                57.67 &
                70.39 &
                4.24 &
                9.10 &
                7.88 &
                14.43 &
                15.01 &
                14.77 &
                45.63 &
                62.41 &
                16.15 &
                19.33 \\
            \hline
                \Block{}{\textcolor{gray}{Supervised}} &
                \textcolor{gray}{CodeT5} &
                \textcolor{gray}{None} &
                \textcolor{gray}{78.49} &
                \textcolor{gray}{73.41} &
                \textcolor{gray}{82.40} &
                \textcolor{gray}{78.49} &
                \textcolor{gray}{73.41} &
                \textcolor{gray}{82.40} &
                \textcolor{gray}{63.23} &
                \textcolor{gray}{28.11} &
                \textcolor{gray}{27.86} &
                \textcolor{gray}{63.23} &
                \textcolor{gray}{28.11} &
                \textcolor{gray}{27.86} &
                \textcolor{gray}{72.26} &
                \textcolor{gray}{85.83} &
                \textcolor{gray}{37.46} &
                \textcolor{gray}{39.49} \\
            \midrule
    \end{NiceTabular}
    }%
\end{table*}
